Multi-Channel Speech Denoising for Machine Ears

This work describes a speech denoising system for machine ears that aims to improve speech intelligibility and the overall listening experience in noisy environments. We recorded approximately 100 hours of audio data with reverberation and moderate environmental noise using a pair of microphone arrays placed around each of the two ears and then mixed sound recordings to simulate adverse acoustic scenes. Then, we trained a multi-channel speech denoising network (MCSDN) on the mixture of recordings. To improve the training, we employ an unsupervised method, complex angular central Gaussian mixture model (cACGMM), to acquire cleaner speech from noisy recordings to serve as the learning target. We propose a MCSDN-Beamforming-MCSDN framework in the inference stage. The results of the subjective evaluation show that the cACGMM improves the training data, resulting in better noise reduction and user preference, and the entire system improves the intelligibility and listening experience in noisy situations.

==> app.tex <==
The code, data, and all other materials, that are related to this project and can be used to reproduce the same results, are stored at {\color{blue}\href{https://drive.google.com/corp/drive/folders/1ZmO-5aev0S1iM5SxcOicfl2fUiKVDcdV}{Drive for Wolverine Core}} and {\color{blue}\href{https://source.corp.google.com/piper///depot/google3/experimental/googlex/wolverine/multichannel_enhancement/}{Code Search}}.

\subsection{Method}
\subsubsection{cACGMM for preprocess the data}
The {\color{blue}\href{https://drive.google.com/corp/drive/folders/1Qdz269nqpZ_VNG3Jmaw9NS8cZvO5SZKo}{cACGMM Code}} removes noise in speech recordings on the local cloudtop. The code is based on the {\color{blue}\href{https://github.com/fgnt/pb_bss}{Implementation}}. {\color{blue}\href{https://drive.google.com/corp/drive/folders/1XSe5avjn2wyEnT6VOsHWZhWPnik4UFh0}{Code and Audio Examples}} will plot the same figure 2.

\subsubsection{DNN training}
{\color{blue}\href{https://source.corp.google.com/piper///depot/google3/experimental/googlex/wolverine/multichannel_enhancement/basic_mc_tasnet/}{Basic MC-TasNet}} code for training the model is at code search. The major body of the code is borrowed from {\color{blue}\href{https://source.corp.google.com/piper///depot/google3/audio/hearing/separation/models/basic_tasnet/}{Basic TasNet}} from the sound understanding group.

\subsubsection{Inference}
{\color{blue}\href{https://source.corp.google.com/piper///depot/google3/experimental/googlex/wolverine/multichannel_enhancement/run_inference/}{Inference and Save Data}} run inference and save all intermittent signals. {\color{blue}\href{https://colab.corp.google.com/drive/1zU7l2UE-KSFA6p69xfUCAbzK9Hj7vtRP#scrollTo=7hifpkXk6ATc}{Inference Demo in Colab}} is also stored at {\color{blue}\href{https://drive.google.com/corp/drive/folders/1ZmO-5aev0S1iM5SxcOicfl2fUiKVDcdV}{Drive}}.



\subsection{Experiment configurations}
\subsubsection{Data recordings}
Please contact Kyle Hoefer (@hoefer) for details.

\subsubsection{Acoustic scene generation}
{\color{blue}\href{https://source.corp.google.com/piper///depot/google3/experimental/googlex/wolverine/data_generation/}{Acoustic Scene Generator}} code is provided by Mathieu Parvaix (@parvaix). {\color{blue}\href{https://source.corp.google.com/piper///depot/google3/experimental/googlex/wolverine/multichannel_enhancement/acoustic_scene_generation/}{Configuration YAML File}} in this project can be found at code search.\\

\subsubsection{Subjective evaluation}
For experiment 1, the surveys (five groups) can be found at {\color{blue}\href{https://survey.alchemer.com/s3/6539962/SoundQuality-T1}{Survey1}, \href{https://survey.alchemer.com/s3/6540119/SoundQuality-T2}{Survey 2}, \href{https://survey.alchemer.com/s3/6541428/SoundQuality-T3}{Survey 3}, \href{https://survey.alchemer.com/s3/6542845/SoundQuality-T4}{Survey 4}, \href{https://survey.alchemer.com/s3/6543638/SoundQuality-T5}{Survey 5}}. The {\color{blue}\href{https://drive.google.com/corp/drive/folders/1WYjBR_6rs-0ZozcX35MyyUoVzWX4yGq5}{Audio Examples}} and the {\color{blue}\href{https://drive.google.com/corp/drive/folders/16xWtSbIbGO44skH-V5S4Kpz-bkEBkIOC}{Responses in CSV}.} collected from the subjects can be found at {\color{blue}\href{https://drive.google.com/corp/drive/folders/16xWtSbIbGO44skH-V5S4Kpz-bkEBkIOC}{Drive}.} For experiment 2, the survey can be found at {\color{blue}\href{https://survey.alchemer.com/s3/6548211/SpeechQuality-Comparison}{Survey 6}}. The {\color{blue}\href{https://drive.google.com/corp/drive/folders/1q7eHslBnNzM0NER9IGTUkdxGDQ5CNQnn}{Audio Examples}} and the {\color{blue}\href{https://drive.google.com/corp/drive/folders/1p5EqUPZO-qX5mhJllh_j2Yh87ol_0SDj}{Responses in CSV}} collected from the subjects can be found at {\color{blue}\href{https://drive.google.com/corp/drive/folders/1p5EqUPZO-qX5mhJllh_j2Yh87ol_0SDj}{Drive}.}


\subsection{Results and discussions}
\subsubsection{Plotting}
For experiment 1, the {\color{blue}\href{https://drive.google.com/corp/drive/folders/16xWtSbIbGO44skH-V5S4Kpz-bkEBkIOC}{Jupyter Notebook}} will plot the same figure 3.

\noindent For experiment 2, the {\color{blue}\href{https://drive.google.com/corp/drive/folders/1p5EqUPZO-qX5mhJllh_j2Yh87ol_0SDj}{Jupyter Notebook}} will plot the same figure 4.


\subsection{Conclusion}
\subsubsection{Final report}
The {\color{blue}\href{https://docs.google.com/presentation/d/1yh5zCGiFuJOSOAuKCowVk7TSwirxqBX68zk37frpFI4/edit?usp=sharing}{Final Report}} can be found at the {\color{blue}\href{https://drive.google.com/corp/drive/folders/1ZmO-5aev0S1iM5SxcOicfl2fUiKVDcdV}{Drive}}.






==> data_collection_cache.tex <==
\subsection{Data collection}
\label{dc}
We collected a database of in-room, on-device acoustic recordings to provide a collection of speech and ambient sound samples to be used in generating sound mixtures for analysis.
Each sample has the real room acoustics, both reverb and background noise.

The room in which acoustic data is recorded has the dimensions of 7.5 (length) x 3.5 (width) x 3 (height) meters. One length-wise wall is made up of glass with white boards covering the opposing side. The width-wise walls are made up of a white board and television. The ceiling is grated aluminum with five inch wide lights stretching across the length of the room, while the floor is carpeted.

A Bruel and Kjaer Type 4128-C Head and Torso Simulator (HATS) is placed in the center of the room on a motorized turntable, which sits atop a wooden table that spans across the majority of the room length-wise. For the purposes of this experiment, we used a proprietary array of $N$ microphones around each of the two ears, giving us a total of $2N$ signals from which to extract the most intelligible signal. Surrounding the HATS are six Genelec 8020D four inch Powered Studio Monitors for playback audio sources. The monitors are placed at varying azimuths and distances from the HATS, as well as varying elevations from the ground. All monitors are facing directly towards the HATS in the center of the room. All possible monitor azimuth values range from 0 to 360\textdegree, with distance and elevation values ranging from one to three meters in one meter increments. Once placed, the monitor locations are fixed and do not change for the given room.

Playback source data utilizes the entirety of the Freesound Dataset 50k (FSD50k) \cite{eduardo_fonseca_2020_4060432}, and LibriSpeech data set \cite{7178964}. Both data sets are kept split by their corresponding development and evaluation subsets. For proper generation of sound mixtures post-recording, the database utilizes the two hundred sound classes of the FSD50k data set, while the LibriSpeech data set is labeled as the target 'non-user speech.' These sound class names are saved for each playback file, and passed along to be written in the metadata when the specific file is chosen to be played out of a monitor. Files undergo preprocessing before playback, including being re-sampled to 48kHz, removing silence from the beginning and end of the file, and level calibration so that the file's dBSPL at the monitor's source is as close as possible to a real-world example. The target dBSPL values for each sound class have a random variance of $\pm 5$ dBSPL.

A playback file is chosen and a random monitor assigned, simultaneously emitting the audio data and recording through the microphone arrays. Upon completion, a multi-channel 48kHz, 32-bit floating point audio file and its associated metadata are saved. The metadata notates the azimuth, distance, and elevation of the chosen playback monitor, as well as the playback file's sound class. Once saved, the motorized turntable rotates five degrees clockwise. The updated turntable rotation is saved, and used in conjunction with the fixed monitor position for reporting the next playback file's azimuth. This ensures the reported azimuth value is always the angle of the monitor relative to the front-facing direction of the HATS. This process is run for both FSD50k and LibriSpeech development and evaluation sets, repeated until the specified number of recording hours per playback sources are met.


==> introduction_old.tex <==
Environmental noise corrupts speech signals. This corruption degrades speech intelligibility and quality and thus hinders human communication in noisy environments. Speech enhancement aims to reduce the background noise in a speech signal and thus improve human hearing. Given its importance, speech enhancement has been actively studied for decades \cite{boll1979suppression, ephraim1984speech, cohen2001speech,gannot2001signal}. In recent years, supervised learning with deep neural network (DNN) has achieved noticeable performance in speech enhancement tasks \cite{xu2013experimental,weninger2015speech}. Supervised learning methods require a large amount of labeled data to train the DNNs. In the speech enhancement task, the labeled data is pair of the observed noisy signal and the target clean signal. The datasets for speech enhancement training are usually created by simulation. This has two advantages, on one hand, it's an effortless task to create an arbitrary amount of data with diverse speakers, all possible categories of sound sources in the background, and various room conditions; on the other hand, we can have access to ground-truth reference, which is essential for supervised learning. However, applying DNNs trained to simulated data on real recordings can cause data mismatch. There is still a difference between the simulated signal and real recording received by microphones due to the complex transmission model of the room, which might be an artificial signal that would allow the DNN to "cheat". Moreover, the simulated data cannot capture the acoustic characteristics and geometry of microphone arrays of a specific device accurately, which is not optimal for developing the enhancement model for a specific hearing device. Therefore, developing models that rely on real recordings is desired. 

However, the biggest challenge for such development is the lack of access to clean oracle signals. Therefore, several unsupervised training methods using only observed noisy speech signals have been proposed. A general category of approaches utilize spatial information to cluster sound sources in the space.  The posterior cluster labels can be used either as masks to separate sources or as pseudo-target to train models \cite{tzinis2019unsupervised,seetharaman2019bootstrapping,drude2019unsupervised,togami2020unsupervised,nakagome2020mentoring} such as deep clustering \cite{hershey2016deep} in a supervised manner. The unsupervised spatial clustering methods include k-means clustering on the inter-channel phase difference \cite{tzinis2019unsupervised}, Gaussian mixture model (GMM) \cite{seetharaman2019bootstrapping}, the complex angular-central Gaussian mixture model (cACGMM) \cite{drude2019unsupervised}, and local Gaussian model (LGM) \cite{togami2020unsupervised}. The mentoring-reverse mentoring mechanism is further introduced to improve LGM \cite{nakagome2020mentoring}. However, these clustering based methods can degrade severely in challenging conditions where spatial features are smeared by room reverberance and strong background noise, especially diffuse noise with no distinct directional features. If there are too many disatractors present, accurate clustering can be difficult without knowing the number of clusters in prior. Moreover, the performance of clustering based methods is sensitive to initialization. 

In this paper, we design a speech denoising system for a hearing device aiming to reduce noise and thus improve intelligibility and quality of the speech with strong environmental noise. We use a specific hearing device to record a considerate amount of recordings with reverberation and moderate background noise and develop the system on these real recordings. This is advantageous because 1) it's real data so the training and testing are more realistic, 2) it includes all the complexities of real room reverberations, and 3) it is less expensive to collect since we can use real rooms and don't need anechoic or special recording rooms. To train the model, we mix recordings of speech and other categories of sounds into mixtures simulating adverse acoustic environments requiring speech enhancement to improve listening. Because the speech recordings can contain environmental noise such as air conditioners and people in the room, we apply the unsupervised method, cACGMM, on the speech recordings to extract the cleaner speech components to serve as the learning target. Since the noise in the speech recordings is moderate, the cACGMM can robustly capture the primary directional speech signals, which results in a reliable pseudo-target. In the inference stage, we use a multi-channel speech enhancement system which comprises DNN, MVDR beamforming, and DNN sequentially to denoise the signals. We perform extensive subjective listening test on the processed signals and show the architecture can improve the intelligibility and subjects would like to use processed signals to improve their listening.

% Malcolm: I think you want to emphasize up front that we are working with real recordings, with reverberation and background noise. This is advantageous because 1) it's real data so the training and testing are more realistic, 2) it includes all the complexities of real room reverberations, and 3) it is less expensive to collect since we can use real rooms and don't need anechoic or special recording rooms.  On the other hand, the data is noisy because there are air conditioners and other environmental noise. Our task in this paper is to remove the background noise so we have better training data for a conventional multi-channel speech enhancement system. 

The rest of the paper is organized as follows. We introduce the framework in Section~\ref{sec:method}, present the data collection and experiment configurations in Section~\ref{sec:config}, analyze the experiment results in Section~\ref{sec:result}, and conclude the paper in Section~\ref{sec:conclusion}.

% Malcolm says: Might be good to have an explicit bullet list of the stages: 1) caCGMM (for preprocessing the training data), 2) MSDN, 3) MVDR, 4) MSDN. You could also put section points in the bullet items.

\begin{figure*}[!t]
    \centering
    \includegraphics[width=2.0\columnwidth]{Figures/diagram.pdf}
    \caption{(A) A diagram of the training process for the speech denoising neural network. A speech recording and three distractor recordings are mixed together to form the noisy mixture. cACGMM is applied on the speech to produce the pseudo-target for training the neural network. (B) A diagram of the inference process of the entire system. The neural network estimates a spectral mask of speech for MVDR-beamforming. We shift one-hot vector $\vec{u}$ to generate multi-channel beamforming output sent to the same neural network again. We re-mix beamforming output and DNN output using a gate $\alpha$ to balance speech distortion and noise reduction.}
    \label{fig:arch}
\end{figure*} 

% Malcolm: in B, I'd switch the top and bottom lines on the left so the multidimensional signal go straight through (put the MSDN box on the bottom.) You might also want to use arrows or bold lines to indicate multidimensional signals.





==> method_old.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=2.0\columnwidth]{Figures/diagram.pdf}
    \caption{Overview of speech denoising system in the training stage (A) and inference stage (B). Blue block denotes the same neural network.}
    \label{fig:arch}
\end{figure*}

% (A) A diagram of the training process for the speech denoising neural network. A speech recording and three distractor recordings are mixed together to form the noisy mixture. cACGMM is applied on the speech to produce the pseudo-target for training the neural network. (B) A diagram of the inference process of the entire system. The neural network estimates a spectral mask of speech for MVDR-beamforming. We shift one-hot vector $\vec{u}$ to generate multi-channel beamforming output sent to the same neural network again. We re-mix beamforming output and DNN output using a gate $\alpha$ to balance speech distortion and noise reduction.


% Given a database that contains M-channel recordings of speech and non-speech, we create the sound mixture $\vec{Y} = \vec{S} + \sum_{i=1}^p{\vec{N}_i}$. Each mixture $\vec Y \in \mathbb{C}^{M \times T \times F}$ contains one speech source $\vec S \in \mathbb{C}^{M \times T \times F}$ and up to p non-speech sources $\vec N \in \mathbb{C}^{M \times T \times F}$, where T, F denotes time frames and frequency bins, respectively, in the short-time Fourier transform domain. Because $\vec{S}$ is a far-field recording which contains much environmental noise, using $\vec{S}$ as the learning target is not optimal. We first apply the unsupervised clustering model, cACGMM, on $\vec{S}$ to estimate a time-frequency mask to extract the cleaner speech signal $\vec{\hat{S}}$ that is used as the pseudo-target to train the speech denoising DNN. The DNN takes $\vec{Y}$ as input and estimates a time-frequency mask to predict $\vec{\hat{S}}$. Then, we employ mask-based MVDR beamforming to enhance the speech signal. Finally, we send the beamformed output to exactly the same DNN again to remove the residual noise. Figure~\ref{fig:arch} shows the proposed method for training and inference. 

Figure 1 shows an overview of the proposed method for training and inference. During training we use cACGMM to generate a better target to train a conventional multi-channel speech denoising network (MCSDN).  In inference we combine the pretrained MCSDN with beam forming and then a fraction of the output from another instance of the same MCSDN. 

\subsection{Complex angular central Gaussian mixture model}
\label{gmm}
Give the recording $\vec{s}$, we use the Complex Angular Central Gaussian Mixture Model (cACGMM) to isolate the speech source $\hat{\vec{s}}$ and remove noisy sources from unwanted direction. In the short-time Fourier transform domain, cACGMM models the directional observations $\vec{Z}_{t,f} = \frac{\vec{S}_{t,f}}{||\vec{S}_{t,f}||}$ with a Gaussian mixture model,

\begin{align}
    p(\vec{Z}_{t,f};\Theta_f) = \sum_{k=1}^K{\alpha^{k}_{f}\mathcal{A}(\vec{Z}_{t,f}; \vec{B}_{f}^{k})},
\end{align}
where $\Theta_f = \{\alpha^{k}_{f},\vec{B}_{f}^{k} \forall k \}$ denotes the model parameters, $\{\alpha^{k}_{f}\forall k \}$ is a set of k mixture weights, which are probabilities that sum to 1. $\mathcal{A}(\vec{s}_{t,f}; \vec{B}_{f}^{k})$, a complex augular Central Gaussian (CACG) distribution, models the distribution of $\vec{Z}_{t,f}$ for the k-th signal component in the mixture model,

\begin{align}
    \mathcal{A}(\vec{Z}_{t,f}; \vec{B}_{f}^{k}) = \frac{(D-1)!}{2\pi^{D}\text{det}(\vec{B}_{f}^{k})}\frac{1}{(\vec{Z}_{t,f}^H(\vec{B}_{f}^{k})^{-1}\vec{Z}_{t,f})^D}.
\end{align}
Model parameters $\Theta_f$ are estimated by the Expectation-Maximization (EM) algorithm. The posterior probability of $\vec{Z}_{t,f}$ belonging to class k is:
\begin{align}
    \Gamma_{t,f}^k = \frac{\alpha^{k}_{f}\mathcal{A}(\vec{Z}_{t,f}; \vec{B}_{f}^{k})}{\sum_{k=1}^K{\alpha^{k}_{f}\mathcal{A}(\vec{Z}_{t,f}; \vec{B}_{f}^{k})}}.
\end{align}

Since cACGMM models each frequency independently, there can be a frequency permutation problem \cite{sawada2007measuring}, i.e., the same index k in different frequency bins point to different sources. The problem is addressed by permutation alignment \cite{sawada2007measuring}.

Finally, we use $\Gamma^k$ as the masks to separate sources. The recording of speech usually has a high signal-to-noise ratio, so we can calculate the similarity between the original recording $\vec{S}$ and each separated source to determine the enhanced speech. We only keep the enhanced speech $\hat{\vec{S}}$ as the pseudo-target to train DNNs,
\begin{align}
    \hat{\vec{S}} = \vec{S} \odot \Gamma^s,
\end{align}
where $\odot$ denotes element-wise multiplication.


\subsection{Multi-channel speech denoising network}
\label{dnn1}
In order to exploit both the spectral-temporal and spatial information, we concatenate the log power spectrogram of the reference channel signal and inter-channel phase differences (IPDs) between the reference channel and other channels as input features. Sound sources from the same direction should have the same IPDs in each frequency band, so IPDs indicate which T-F bins belong to the same directional source. Specifically, we calculate \text{sinIPD} and \text{cosIPD} as inter-channel features.

Then, we apply the temporal convolutional network (TCN) \cite{bai2018empirical,luo2019conv} on the input feature to estimate the speech mask $\vec{M}^{s} \in \mathbb{R}^{F \times T}$. TCN consists of stacks of 1-D convolutional layers with dilation in the temporal dimension, which results in a larger receptive field to capture long-term contextual information. The training objective is defined as:
\begin{align}
    \mathcal L = |\vec{Y} \odot \vec{M}^s - \vec{\hat{S}}|
\end{align}



\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\columnwidth]{Figures/spec_gray.pdf}
    \caption{The cACGMM extracts a cleaner speech (right) from the recording (left) as the training target. The red rectangle shows an instance where the background noise is removed.}
    \label{fig:p2}
\end{figure} 


\subsection{Mask-based MVDR beamforming}
\label{beamforming}

To attenuate the interferences while introducing minimum nonlinear speech distortions, we perform MVDR beamforming to enhance the speech signal in the frequency domain. The signals from all M microphones are represented as:
\begin{align}
    \vec{Y}_{t,f} = [\vec{Y}_{1,t,f}, \vec{Y}_{2,t,f}, \dots, \vec{Y}_{m,t,f}]^{T},
\end{align}
where T denotes non-conjugate transposition. The beamformer estimates a linear filter $\vec{w}_f \in \mathbb{C}^{M}$ in each frequency $f$ and applies $\vec{w}_f$ to $\vec{Y}_{t,f}$ to generate the enhanced output $\vec{BF}_{t,f} \in \mathbb{C}^{F}$,
\begin{align}
    \vec{BF}_{t,f} = \vec{w}_f^H \vec{Y}_{t,f},
\end{align}
where H denotes conjugate transposition. After optimization with a constraint that minimizes the power of noise without distorting the target speech, one solution is:
\begin{align}
    \vec{w}_{f} = \frac{(\vec{\Phi}_{f}^{n})^{-1}\vec{\Phi}_{f}^s}{\text{Trace}({(\vec{\Phi}_{f}^{n})^{-1}\vec{\Phi}_{f}^s})}\vec{u},
\end{align}
where $\vec{\Phi}_{f}^{n}$ and $\vec{\Phi}_{f}^{s}$ are the covariance matrices of the noise and speech, respectively, and $\vec{u}$ is a one-hot vector indicating the reference channel. The mask-based MVDR beamforming uses the mask $\vec{M}_{t,f}^s$ from the DNN to estimate $\vec{\Phi}_{t,f}^{s}$ and $\vec{\Phi}_{t,f}^{n}$,
\begin{align}
    &\vec{\Phi}_{f}^{s} = \frac{1}{\sum_{t}{\vec{M}_{t,f}^s}}\sum_{t}{\vec{M}_{t,f}^s} \vec{Y}_{t,f}\vec{Y}_{t,f}^{H} \\
    &\vec{\Phi}_{f}^{n} = (\frac{1}{T}\sum_{t} \vec{Y}_{t,f}\vec{Y}_{t,f}^{H}) - \vec{\Phi}_{f}^{s}
\end{align}

\subsection{Post-enhancement after beamforming}
\label{dnn2}
The MVDR beamforming effectively keeps speech free of nonlinear distortion, which is essential for good perceptual quality of speech in communication. However, the MVDR beamforming cannot cancel all interference, especially when some are close in space to the speech source. To reduce the residual noise, $\vec{BF}_{t,f}$ is sent to a post-enhancement module. Some work introduces another neural network as the post-enhancement module \cite{wang2021multi}. However, adding a new neural network increases the size of the whole model, which is challenging for its deployment on hardware with limited capacities, such as hearing aids. To save model size and take advantage of both spectral and spatial information, the multi-channel speech enhancement network in Section~\ref{dnn1} is re-used here. 

To extend the single-channel beamforming output to a multi-channel single, $\vec{BF} \in \mathbb{C}^{M \times T \times F}$, we stack the beamforming output on each channel $<\vec{BF}_{1}, \vec{BF}_{2}, \dots, \vec{BF}_{m}>$ by simply shifting the one-hot vector $\vec{u}$ without introducing any new computation. Finally, the multi-channel speech enhancement network takes $\vec{BF}$ as input and estimates a speech mask $\hat{\vec{M}}^s \in \mathbb{C}^{T \times F}$ for the beamformed output:
\begin{align}
    \overline{\vec{S}} = \hat{\vec{M}}^s \odot \vec{BF}
\end{align}
we can view the pipeline in this way: the first time-frequency mask estimation is for mask-based beamforming that results in a less noisy mixture, then the second mask estimation is to extract the speech from the noisy mixture. 

However, using the spectral mask estimated by neural networks to extract speech will inevitably cause non-linear speech distortion, which is undesirable for human listening. We can balance the noise reduction and speech distortionless by mixing the beamforming output and the neural network output using a gate $\alpha \in [0, 1]$,
\begin{align}
    \widetilde{\vec{S}} = \alpha \cdot \vec{BF} + (1-\alpha) \cdot \overline{\vec{S}}.
\end{align}



==> rebuttal.tex <==
\subsection{Review 1 and our rebuttal}

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.9\columnwidth]{Figures/pic1.png}
    \label{fig:r1}
\end{figure}

We thank the reviewers for taking the time to read our manuscript and for the constructive feedback. \\
~\\
Q1: This reviewer cannot find theoretical nor practical improvements from the method proposed (cACGMM) in [9] in terms of the first contribution (applying cACGMM to extract a clean speech signal from recorded signals with a small amount of noise).
~\\
A1: Our study does show that cACGMM improves the quality of training data coming from real recordings. We performed an ablation study to demonstrate the effectiveness of cACGMM to improve the training dataset. One challenge when using real recorded sounds as a training target is that the sounds contain background noise, so the supervised models cannot learn to completely denoise the recordings. The unsupervised method, cACGMM, can extract a cleaner speech from the noisy recording to improve supervised training. We tested two MCSDN models trained with and without cACGMM, respectively, and asked the subjects to compare and rate them for noise reduction and listening improvement. As shown in Figure 4, the model trained using the cleaner target speech provided by cACGMM results in better noise reduction and thus better listening improvement. This demonstrates that cACGMM can improve the quality of training data coming from practical real recordings. \\ 

~\\
Q2: The second technique is quite similar to [16]. Although this paper further proposes some techniques to reduce computational cost and leverage additional noise recordings, their effectiveness is not validated in the experiments. Furthermore, the same DNNs are used twice to reduce the required memory at the time of inference. The experiments, however, did not investigate these points.
~\\
A2: The only similar point to [16] is using time-frequency masks to estimate MVDR weights. It's a popular method to combine DNNs and conventional beamforming methods in recent years, so we adopted the same technique and cited some representative papers, including [16]. 

One of our contributions was to propose to use the same multi-channel speech denoising network (MCSDN) as a post enhancement neural network to further improve the MVDR outputs. Recent papers [17, 18] train another single-channel speech enhancement network for post enhancement. However, adding a new neural network increases the size of the system, which is undesirable when deploying on hardware with limited capacities, such as hearing aids. To our best knowledge, our paper is the first one that proposes to use the duplicated multichannel DNN for post enhancement. We need to clarify, we don't claim the duplicated MCSDN can reduce the required (computational) cost at the time of inference. The point of the duplicated (MCSDN) network is to simplify the implementation and save model parameters. We want to demonstrate that this simplification is possible and works as well.

Also, we validated the effectiveness of the duplicated MCSDN in the first experiment as shown in Fig. 3 and gave full discussion in section 5. The duplicated MCSDN, following the beamformer, reduces the residual noise noticeably but still lifts speech distortion slightly. It does not affect intelligibility and achieves slightly better listening improvement than beamforming. All metrics at the output of the duplicate MCSDN are significantly better than the first MCSDN.


~\\
Q3: Although this reviewer recognizes the importance of the subjective evaluation, the effectiveness of the proposed method is unclear in the results of the subjective evaluation. In all metrics, cACGMM outperformed the proposed method in terms of median performance.
~\\
A3: Thanks for your feedback. Sorry for the confusion, and we could have presented Fig.3 in a better way. In Fig.3, the cACGMM output, which we label as pseudo-target, is processed from moderately noisy recordings and used as the training target of the MCSDN. Differently, MCSDN, MVDR, MVDR-MCSDN, and Re-mix were tested on the extreme noisy mixtures (mix of four noisy recordings) to examine their enhancement performance. So, it's expected that the cACGMM output achieves the highest mean scores in all aspects. The reason we put cACGMM here is to show that it is able to produce good quality signals to serve as the training target for MCSDN. [We have modified the legend of Fig.3 to make this point more salient.]\\

~\\
Q4: In addition, performances of a supervised baseline or other unsupervised methods should be investigated.
~\\
A4: Thanks for your good suggestion. The MCSDN, labeled in blue in Fig.3, is the supervised baseline although its training target is from cACGMM. Pure unsupervised methods, such as cACGMM, CGMM, Kmeans, failed enhancing speech in extreme noisy mixtures in our setting. Pure supervised methods, e.g., MCSDN trained without cACGMM, had very poor performance because the training target contains noticeable noise. So, we didn't include them in the subjective evaluation. We agree it's helpful to compare cACGMM with other unsupervised methods in our system, however, performing sufficient subjective evaluation takes effort. Designing efficient evaluation methods and giving more detailed comparisons are future work.

This paper proposed to combine unsupervised learning, supervised learning, and beamforming techniques for developing an enhancement model using real-recorded sounds. The main focus of this paper is to investigate the effectiveness of each component, especially the unsupervised model cACGMM, on improving human listening experience, which is helpful for future work to design hearing aids using real recordings. We believe this is the uniqueness and big contribution of this paper. 



\clearpage
\subsection{Review 2 and our rebuttal}

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\columnwidth]{Figures/pic2.png}
    \label{fig:r2}
\end{figure}

~\\\\\\\\\\\\\\\\\\\\
Thank you for your constructive comments and support. We have corrected the typos. The reviewer also questions why the medians (red lines) are aligned to discrete values (integers) in Fig. 3. Because the test was a simplified version of multiple stimuli with hidden reference and anchor (MUSHRA), the subjects rated all aspects of each processed speech sample on a scale with the following labels: bad (1), poor (2), fair (3), good (4), and excellent (5). All ratings are discrete value, so the median is also a discrete value, but the mean can be a non-discrete value.

We agree the title of the paper is too broad and not descriptive of our contribution.  We will endeavor to change the title, with the organizer's permission, to "Multi-Channel Speech Denoising Using an Unsupervised Method to Clean the Training Data". 




\clearpage
\subsection{Review 3 and our rebuttal}

\begin{figure}[!h]
    \centering
    \includegraphics[width=1.0\columnwidth]{Figures/pic3.png}
    \label{fig:r3}
\end{figure}

~\\\\\\\\\\\\\\\
We thank the reviewer for taking the time to read our manuscript and for the constructive feedback and support. 
The reviewer notes that testing and training are carried out in the same room, which can cause overfitting to a particular room. This is a worthy concern. We agree with the reviewer that including the results from different rooms would be helpful. However, current experiments don't weaken the focus and conclusions in this paper. 

We propose to apply cACGMM on individual recordings to extract clean speech signals to serve as the target for learning, which significantly improves the training dataset. The cACGMM, as an unsupervised model, doesn't make any assumptions about the rooms. And in Figures 3 and 4, we show the effectiveness of the cACGMM. The only component in our framework that can overfit the rooms is the multi-channel speech denoising network (MCSDN). However, in this paper, our focus is not a new neural network; instead, we adopt TasNet that has shown success, including dealing with reverberation across different rooms, in many papers. The MCSDN can be any other effective neural networks, and choosing which network is not the focus of this paper. The paper's focus is to investigate the effectiveness of each component, including the first DNN, MVDR, and the second DNN, on improving human listening experience. This is helpful for future work to design hearing aids using real recordings. We do not believe this ablation study is weakened by testing in the same room.





==> result_old.tex <==
Figure~\ref{fig:r4} compares different models in intelligibility, noise reduction, free of speech distortion, and overall listening improvement. First of all, the cACGMM achieves the highest mean scores in all perspectives. More than 75\% scores are no less than 4 in the rating of intelligibility, noise reduction, and overall listening improvement, respectively. That is because the cACGMM is applied on the speech recordings with moderate background noise, so the performance of the cACGMM is good and stable. We notice the score for 'free of distortion' is a bit worse, perhaps because cACGMM estimates a probabilistic time-frequency mask through spatial clustering, which may introduce nonlinear distortion. Overall, the signals from cACGMM have decent performance in the listening test, so it is appropriate to use it as the learning target to train the DNN model.

It should be noted that human can attend to the source of interest during the presence of multiple stimuli thanks to the cocktail part effect. So, some subjects are still able to recognize what the speaker is saying in some examples with low SNRs. Overall, the unprocessed speech signals achieve the lowest intelligibility score because the strong background noise makes the speech much less intelligible. As shown in the first figure, all models improve intelligibility. Not surprisingly, the DNN model has a high score for noise reduction because of the modeling power of nonlinear models. However, this can cause severe speech distortion. If the mixture is too noisy, the model may also filter out speech components when it removes the noise. So, the DNN only gains slight intelligibility improvement. The MVDR beamforming and MVDR beamforming-DNN have similar intelligibility scores. The MVDR beamforming using linear filters avoids nonlinear distortion but sacrifices the capability of canceling noise. The second DNN, following the beamforming, further filters out the residual noise but still lifts speech distortion. However, the beamforming output is less noisy than the unprocessed signals, making it easier for the second DNN to denoise. Therefore, the scores of the second DNN for noise reduction and free of distortion are both better than the ones of the first DNN. When 20\% of the beamforming output and 80\% of the second DNN output are re-mixed as a new signal, we see it significantly improves the intelligibility score. It's because both distortionless and noise reduction are important factors for intelligibility. The beamforming output can compensate for the distorted components in the DNN. We notice that the score for the re-mixed one is even close to the pseudo-target from cACGMM.  The re-mix model achieves the best core for listening improvement. Some subjects mentioned they felt comfortable when the sound contained a little background noise. One explanation is that it is more realistic than pure, clean sound or over-denoised sound; moreover, the beamforming output can compensate for the lost components, especially high frequency, which is essential for intelligibility. 

Figure~\ref{fig:r5} compares the re-mix model with the DNNs trained without and with the cACGMM. We see the model trained using cleaner target speech processed by the cACGMM results in better noise reduction and thus better listening improvement. This proves the cACGMM can help improve the quality of training data coming from real recordings. The mean number 4.11 and 4.05 are slightly better than the scores 3.71 and 3.91 in Figure~\ref{fig:r4} probably because the subject were not perceptually influenced by the processed signals from DNNs and pseudo-target when they only compared models w/ and w/o cACGMM.


% [Malcolm: I can't find the source of the results figure.  Why do the bars all start and end on integer values?  Otherwise, results look intriguing.  But it's hard to tell.  Do we need more subjects?]

